Efficient stochastic optimisation by unadjusted Langevin Monte Carlo. Application to maximum marginal likelihood and empirical Bayesian estimation

Stochastic approximation methods play a central role in maximum likelihood estimation problems involving intractable likelihood functions, such as marginal likelihoods arising in problems with missing or incomplete data, and in parametric empirical Bayesian estimation. Combined with Markov chain Monte Carlo algorithms, these stochastic optimisation methods have been successfully applied to a wide range of problems in science and industry. However, this strategy scales poorly to large problems because of methodological and theoretical difficulties related to using high-dimensional Markov chain Monte Carlo algorithms within a stochastic approximation scheme. This paper proposes to address these difficulties by using unadjusted Langevin algorithms to construct the stochastic approximation. This leads to a highly efficient stochastic optimisation methodology with favourable convergence properties that can be quantified explicitly and easily checked. The proposed methodology is demonstrated with three experiments, including a challenging application to high-dimensional statistical audio analysis and a sparse Bayesian logistic regression with random effects problem.

==> fixed_batch.tex <==
\begin{proof}
  Recall that for any $k \in \N$ we have
  \begin{equation}
    \eta_k =  H_{\theta_k}(X_{k+1}) - \nabla f(\theta_k) = H_{\theta_k}(X_{k+1}) - \pi_{\theta_k}(H_{\theta_k}) \eqsp .
  \end{equation}
  In order to apply \cite[Theorem 2]{atchade2017perturbed} we must show that the following sums converge \as 
  \begin{equation}
    \sum_{k=0}^n \delta_{k+1} \langle \Pi_{\Theta} \parentheseDeux{\theta_k - \delta_k \nabla f(\theta_k) }, \eta_k \rangle \eqsp , \qquad \sum_{k=0}^n \delta_{k+1} \eta_k \eqsp, \qquad \sum_{k=0}^n \delta_{k+1}^2 \|\eta_k \|^2 \eqsp .
  \end{equation}

  Using \eqref{eq:condition_majo_V_fix} we get for any $ n \in \N$, $\expe{\| \eta_n \|^2} \leq 2M_H^2 C_0 \expe{V(X_0)} + 2 \sup_{\theta \in \Theta} \| \nabla f(\theta) \|^2<+\infty$. Thus we obtain for any $n \in \N$,
  \begin{equation}
    \expe{\sum_{k=0}^n \delta_{k+1}^2 \| \eta_k\|^2} \leq \sup_{k \in \N} \expe{\| \eta_k \|^2} \sum_{k=1}^n \delta_k^2 < +\infty\eqsp .
  \end{equation}
  Thus we obtain that \as \ $ \sum_{k=0}^n \delta_{k+1}^2 \|\eta_k \|^2 <+\infty$ .
  % Considering the asymptotic bias we get for any $n \in \N$
  %   \begin{equation}
  %   \eta_n =  H_{\theta_n}(X_n) - \pi_{\gamma_n,\theta_n}(H_{\theta_n}) + \pi_{\gamma_n,\theta_n}(H_{\theta_n}) - \pi_{\theta_n}(H_{\theta_n}) \leq C(1 + V(x)) \sum_{n = 0}^N \delta_n^2 \eqsp .
  % \end{equation}
For any $\theta \in \Theta$ and $ \gamma \in (0, \bgamma)$ we define $\hat{H}_{\gamma, \theta}(x)$ for any $x \in \rset^d$ as 
  $\hat{H}_{\gamma,\theta}(x) = \sum_{k \in \N} K_{\gamma,\theta}^kH_{\theta}(x) - a_{\gamma, \theta}$. We have the following inequality using \eqref{eq:condition_V_fix} for all $\theta \in \Theta$, $\gamma \in (0, \bgamma)$ and $x \in \rset^d$
  \begin{equation}
    \label{eq:poisson_majo}
    \| \poiss{}(x) \| \leq C_1 \log(1/\rho)^{-1} \rho^{-\bgamma} \gamma^{-1} V(x) \eqsp .
  \end{equation}

We recall that $\poiss{}$ satisfies the following fundamental equation for all $\theta \in \Theta$, $\gamma \in (0, \bgamma)$ and $x \in \rset^d$
\begin{equation}
  \label{eq:poisson_eq}
  K_{\gamma,\theta} \poiss{}(x) - \poiss{}(x) =  H_{\theta}(x) -a_{\gamma, \theta} \eqsp .
\end{equation}

Using \eqref{eq:poisson_eq} we have the following equalities for all $k \in \N$
\begin{align}
  \eta_{k} &=  \kernel{k} \poiss{k}(X_{k+1}) - \poiss{k}(X_{k+1}) + a_{\gamma_k, \theta_k} - \pi_{\theta_{k}}(H_{\theta_{k}}) \\
             &= \kernel{k}\poiss{k}(X_k) - \poiss{k}(X_{k+1})\\ & \phantom{aa} + \kernel{k+1}\poiss{k+1}(X_{k+1}) - \kernel{k}\poiss{k}(X_{k}) \\ & \phantom{aa} +  \kernel{k}\poiss{k}(X_{k+1}) - \kernel{k+1}\poiss{k+1}(X_{k+1}) + a_{\gamma_k, \theta_k} - \pi_{\theta_{k}}(H_{\theta_{k}}) \eqsp .
\end{align}

We have that $\eta_k = \eta_k^a + \eta_k^b + \eta_k^c + \eta_k^d$ where 
\begin{equation}
  \left\lbrace \begin{aligned}
      &\eta_{k}^a =  \kernel{k}\poiss{k}(X_k) - \poiss{k}(X_{k+1})\eqsp ; \\ &\eta_{k}^b =  \kernel{k+1}\poiss{k+1}(X_{k+1}) - \kernel{k}\poiss{k}(X_{k}) \eqsp ; \\ &\eta_{k}^c =  \kernel{k}\poiss{k}(X_{k+1}) - \kernel{k+1}\poiss{k+1}(X_{k+1})\eqsp ; \\
    & \eta_k^d = a_{\gamma_k, \theta_k} - \pi_{\theta_k}(H_{\theta_k}) \eqsp .\end{aligned} \right.
\end{equation}
In the rest of the proof we show that the following sums converge
\begin{equation}
  \sum_{k=0}^n \delta_{k+1} \langle \Pi_{\Theta} \parentheseDeux{\theta_k - \delta_k \nabla f(\theta_k) }, \eta_k^i \rangle \eqsp , \qquad \sum_{k=0}^n \delta_{k+1} \eta_k^i \eqsp ,
\end{equation}
where $i \in \lbrace a, b, c,d \rbrace$.

\begin{enumerate}[wide, labelwidth=!, labelindent=0pt, label=(\alph*)]
  \item We have that $(\eta_{k}^a)_{k \in \N}$ is a martingale increment with respect to $\mathcal{F}_k$. Thus using \eqref{eq:poisson_majo} and \eqref{eq:condition_majo_V_fix}  we obtain for any $n \in \N$
    \begin{align}
      \expe{\|  \sum_{k=0}^n \delta_{k+1} \eta_k^a \|^2 } &= \sum_{k=0}^n \delta_{k+1}^2 \expe{ \| \eta_k^a \| ^2} \\ &\leq \sum_{k=0}^n \delta_{k+1}^2 \expe{\CPE{\|\poiss{k}\|^2(X_{k+1})}{ \mathcal{F}_{k}} } \leq C \sum_{k=0}^n \delta_{k+1}^2 \gamma_k^{-2} \eqsp ,
    \end{align}
    The martingales $\sum_{k=0}^n \delta_{k+1} \langle \Pi_{\Theta} \parentheseDeux{\theta_k - \delta_k \nabla f(\theta_k) }, \eta_k^i \rangle$ and  $\sum_{k=0}^n \delta_{k+1} \eta_k^i$ are bounded in $L^2(\Omega, \mathbb{P})$ and thus converge \as .
  \item Summing the second term $\eta_{k}^b$ we apply a discrete integration formula and we obtain for any $n \in \N$
    \begin{align}
      \sum_{k=0}^n  \delta_{k+1} \eta_k^b &= \sum_{k=0}^n \delta_{k+1} \left( \kernel{k+1}\poiss{k+1}(X_{k+1}) - \kernel{k}\poiss{k}(X_k) \right) \\ &= \sum_{k=1}^{n} \left( \delta_{k} - \delta_{k+1} \right) \kernel{k} \poiss{k} (X_{k}) \\ & \phantom{aaaa} + \delta_{n+1} \kernel{n+1} \poiss{n+1} (X_{n+1}) - \delta_1 \kernel{0}\poiss{0} (X_0) \eqsp .
    \end{align}
We have using \eqref{eq:poisson_majo} for any $k \in \N$
\begin{equation}
  \sum_{k=1}^{n} \left| \delta_{k} - \delta_{k+1} \right|\expe{ \kernel{k}\| \poiss{k} (X_{k})\|} \leq C \sum_{k=1}^{n} |\delta_k - \delta_{k+1} |  \gamma_k^{-1}  \eqsp .
\end{equation}
Thus the series $\sum_{k=1}^{n} \left( \delta_{k} - \delta_{k+1} \right) \kernel{k} \poiss{k} (X_{k})$ is \as \ absolutely convergent. On the other side we have that the random variable $ \kernel{n+1} \|\poiss{n+1} (X_{n+1})\| $ is bounded by $\gamma_{n+1}^{-1} M_H \kernel{n+1} \poiss{n+1} V^{1/2}(X_{n+1})$.
Let $\vareps >0$, we have using the Markov inequality and \eqref{eq:condition_majo_V_fix} that 
\begin{equation}
  \sum_{n \in \N} \proba{\delta_n \gamma_n^{-1}K_{\gamma_n,\theta_n}V^{1/2}(X_n) \geq \vareps}  \leq \vareps^{-2} \sum_{n \in \N} \delta_n^2 \gamma_n^{-2} M_H C_0 \expe{V(X_0)} < +\infty\eqsp .
\end{equation}
Using the Borel-Cantelli lemma we get that \as \ $\lim_{n \to +\infty} \delta_n \kernel{n} \poiss{n}(X_n) = 0$.
This concludes for the convergence of $\sum_{k=1}^n \delta_{k+1} \eta_k^b$ using \eqref{eq:condition_cv_fix}. We conclude for the convergence of $\sum_{k=1}^n \delta_{k+1} \langle \Pi_{\Theta} \parentheseDeux{\theta_k - \delta_{k+1} \nabla f(\theta_k)} , \eta_k^b \rangle$, upon noticing that $a_{k+1} = \delta_{k+1} \langle \Pi_{\Theta} \parentheseDeux{\theta_k - \delta_{k+1} \nabla f(\theta_k)}$ satisfies $\| a_{k+1} - a_k \| \leq | \delta_{k+1} - \delta_k|$ using \Cref{assum:f_diff}.

\item We now turn to $\eta_k^c$. We start by giving an upper-bound on $\| \pi_{\gamma,\theta} - \pi_{\gamma',\theta'} \|_{V}$ for $\gamma \geq \gamma' >0$ and, $\theta, \theta' \in \Theta$. Let $n \in \N$ and $f \in \functionspace[]{\rset^d}$ such that $| f |_{V} \leq 1$, we get that for any $x \in \rset^d$
  \begin{align}
    \abs{K_{\gamma,\theta}^nf(x) - K_{\gamma',\theta'}^nf(x)} &= \abs{\sum_{j=0}^{n} K_{\gamma,\theta}^{j }(K_{\gamma, \theta}^{} - K_{\gamma', \theta'}^{}) \defEns{K_{\gamma', \theta'}^{(n-j)}f(x) - \pi_{\gamma',\theta'}(f)}} \\
                                                              &\leq C \sum_{j=0}^{n} \lambda^{(n-j)\gamma}\abs{K_{\gamma,\theta}^{j }(K_{\gamma, \theta}^{} - K_{\gamma', \theta'}^{})V(x)} \\
                                                              &\leq C \sum_{j=0}^{n}  \lambda^{(n-j)\gamma} \Delta(\theta,\theta', \gamma, \gamma') \sup_{k \in \N} \kernel{}^{k} V(x) \leq C \gamma^{-1} \Delta(\theta,\theta', \gamma, \gamma') V(x) \eqsp .
  \end{align}
Let $k \to +\infty$ and since $K_{\gamma,\theta}$ is $V$-ergodic we obtain that for any $\theta, \theta' \in \Theta$ and $\gamma' > \gamma >0$
\begin{equation}
  \|\pi_{\gamma,\theta} - \pi_{\gamma',\theta'} \|_{V} \leq C \gamma^{-1} \Delta(\theta, \theta',\gamma, \gamma') V(x) \eqsp .
\end{equation}
We then have the following inequalities
\begin{align}
  \abs{K_{\gamma, \theta} \poissp{\gamma}{\theta}(x) - K_{\gamma', \theta'} \poissp{\gamma'}{\theta'}(x)} &= \abs{K_{\gamma,\theta} \sum_{n \in \N} \defEns{K_{\gamma,\theta}^nH_{\theta} - \pi_{\gamma,\theta}(H_{\theta})} - K_{\gamma',\theta'} \sum_{n \in \N} \defEns{K_{\gamma',\theta'}^nH_{\theta'} - \pi_{\gamma',\theta'}(H_{\theta'})} } \\
                                                                                                    &\leq \abs{ \sum_{n \geq 1} \defEns{K_{\gamma,\theta}^nH_{\theta} - \pi_{\gamma,\theta}(H_{\theta})} -\sum_{n \geq 1} \defEns{K_{\gamma',\theta'}^nH_{\theta'} - \pi_{\gamma',\theta'}(H_{\theta'})} } \\
                                                                                                    &  
\end{align}
In order to control this quantity we will first control the following for all $\theta, \theta' \in \Theta$, $\gamma, \gamma' > 0$, $f, f'\in \functionspace[]{\rset^d}$, $n \in \N$ and $x \in \rset^d$
\begin{equation}
  K_{\gamma,\theta}^nf(x) - K_{\gamma',\theta'}^n f'(x) = K_{\gamma,\theta}^nf(x) - K_{\gamma',\theta'}^n f(x) + K_{\gamma',\theta'}^n (f(x) - f'(x)) \eqsp .
\end{equation}
We have
\begin{align}
  K_{\gamma,\theta}^nf(x) - K_{\gamma',\theta'}^n f(x) &= \sum_{j=0}^{n-1}\defEns{K_{\gamma,\theta}^j - \pi_{\gamma,\theta}}(K_{\gamma,\theta} - K_{\gamma',\theta'}) \defEns{K_{\gamma',\theta'}^{n-1-j}f(x) - \pi_{\gamma',\theta'}(f)} \\
                                                             & \phantom{aa} + \sum_{j=0}^{n-1}\pi_{\gamma,\theta}\defEns{K_{\gamma',\theta'}^{n-1-j}f(x) - K_{\gamma',\theta'}^{n-j}f(x)} \\
  &=\sum_{j=0}^{n-1}\defEns{K_{\gamma,\theta}^j - \pi_{\gamma,\theta}}(K_{\gamma,\theta} - K_{\gamma',\theta'}) \defEns{K_{\gamma',\theta'}^{n-1-j}f(x) - \pi_{\gamma',\theta'}(f)} \\
                                                             & \phantom{aa} + \pi_{\gamma,\theta}(K_{\gamma',\theta'}^nf(x) - f(x)) \eqsp .
\end{align}
Combining \note{...} and \note{...} we obtain that
\begin{align}
  K_{\gamma,\theta}^nf(x) - K_{\gamma',\theta'}^n f'(x) =  &=\sum_{j=0}^{n-1}\defEns{K_{\gamma,\theta}^j - \pi_{\gamma,\theta}}(K_{\gamma,\theta} - K_{\gamma',\theta'}) \defEns{K_{\gamma',\theta'}^{n-1-j}f(x) - \pi_{\gamma',\theta'}(f)} \\
                                                             & \phantom{aa} + \pi_{\gamma,\theta}(K_{\gamma',\theta'}^nf(x) - f) + K_{\gamma',\theta'}^n(f(x) - f'(x)) \eqsp .
\end{align}

Setting $\tilde{H}_{\theta} = H_{\theta} - \pi_{\gamma,\theta}H_{\theta}$ and $\tilde{H}_{\theta'} = H_{\theta'} - \pi_{\gamma',\theta'}H_{\theta'}$ we get that
\begin{align}
  K_{\gamma,\theta}^n \tilde{H}_{\theta}(x) - K_{\gamma',\theta'}^n \tilde{H}_{\theta'}(x) &=  \sum_{j=0}^{n-1}\defEns{K_{\gamma,\theta}^j - \pi_{\gamma,\theta}}(K_{\gamma,\theta} - K_{\gamma',\theta'}) \defEns{K_{\gamma',\theta'}^{n-1-j}H_{\theta}(x) - \pi_{\gamma',\theta'}(H_{\theta})} \\
                                                                                        & + \pi_{\gamma,\theta}(K_{\gamma',\theta'}^nH_{\theta}(x) - H_{\theta}) + K_{\gamma',\theta'}(H_{\theta}(x) - H_{\theta'}(x) + \pi_{\gamma',\theta'}H_{\theta'} - \pi_{\gamma,\theta}H_{\theta}) \\
                                                                                        &=  \sum_{j=0}^{n-1}\defEns{K_{\gamma,\theta}^j - \pi_{\gamma,\theta}}(K_{\gamma,\theta} - K_{\gamma',\theta'}) \defEns{K_{\gamma',\theta'}^{n-1-j}H_{\theta}(x) - \pi_{\gamma',\theta'}(H_{\theta})} \\
                                                                                        & + \pi_{\gamma,\theta}K_{\gamma',\theta'}^nH_{\theta}(x) + K_{\gamma',\theta'}(H_{\theta}(x) - H_{\theta'}(x) + \pi_{\gamma',\theta'}H_{\theta'}) \\
&=  \sum_{j=0}^{n-1}\defEns{K_{\gamma,\theta}^j - \pi_{\gamma,\theta}}(K_{\gamma,\theta} - K_{\gamma',\theta'}) \defEns{K_{\gamma',\theta'}^{n-1-j}H_{\theta}(x) - \pi_{\gamma',\theta'}(H_{\theta})} \\
  & + (\pi_{\gamma,\theta} - \pi_{\gamma',\theta'})(K_{\gamma',\theta'}^nH_{\theta}(x)-\pi_{\gamma',\theta'}H_{\theta}) + K_{\gamma',\theta'}H_{\theta}(x) - \pi_{\gamma',\theta'}H_{\theta} \\& + K_{\gamma',\theta'}H_{\theta'}(x) - \pi_{\gamma',\theta'}H_{\theta'}
\end{align}
For the first term we obtain
\begin{align}
  \abs{\sum_{j=0}^{n-1}\defEns{K_{\gamma,\theta}^j - \pi_{\gamma,\theta}}(K_{\gamma,\theta} - K_{\gamma',\theta'}) \defEns{K_{\gamma',\theta'}^{n-1-j}H_{\theta}(x) - \pi_{\gamma',\theta'}(H_{\theta})}} &\leq C \Delta(\theta, \theta',\gamma,\gamma') \sum_{j=0}^{n-1}\lambda^{j \gamma} \lambda^{(n-1-j)\gamma'} \\ &\leq C \Delta(\theta, \theta',\gamma,\gamma') n\lambda^{n\gamma} V(x)
\end{align}
For the second term we obtain 
\begin{equation}
  \abs{(\pi_{\gamma,\theta} - \pi_{\gamma',\theta'})(K_{\gamma',\theta'}^nH_{\theta}(x)-\pi_{\gamma',\theta'}H_{\theta})} \leq C \|\pi_{\gamma,\theta} - \pi_{\gamma',\theta'} \|_V \lambda^{n\gamma'} \leq C \Delta(\theta, \theta', \gamma, \gamma') \lambda^{n \gamma'} V(x) \eqsp .
\end{equation}
For the third term we obtain
\begin{equation}
  \abs{K_{\gamma',\theta'}^n(H_{\theta} - H_{\theta'})(x) - \pi_{\gamma',\theta'}(H_{\theta} - H_{\theta'})} \leq C \lambda^{n \gamma'} \| \theta - \theta'\|V(x) \eqsp .
\end{equation}
Combining \note{...} we obtain that
\begin{equation}
  \abs{K_{\gamma,\theta}\poissp{\gamma}{\theta}(x) - K_{\gamma',\theta'}\poissp{\gamma'}{\theta'}(x)} \leq C \parentheseDeux{\delta(\theta,\theta',\gamma, \gamma')\gamma^{-2} + \Delta(\theta,\theta',\gamma, \gamma')\gamma'^{-1} + \| \theta - \theta'\|\gamma'^{-1}}V(x) \eqsp .
\end{equation}
\end{enumerate}
\note{tout faire avec du $V^{1/2}$ car ensuite quand on regarde la différence des theta on sort du H theta}
Combining \note{expe borne} and \note{...} we get that for all $n \in \N$,
\begin{equation}
  \sum_{n=0}^N\delta_n \| \eta_n^c \| \leq  \sum_{n=0}^N C \eqsp .
\end{equation}

\item For $\eta_n^c$ we use \eqref{eq:condition_V_fix} and \eqref{eq:condition_cv_fix} to conclude that $\sum_{k=0}^n \delta_{k+1} \| \eta_k^d \|$ converges.

\valentin{En fait il faudra reprendre la preuve avec l'opérateur matriciel ($A$ chez atchadé). Le premier et le dernier points restent indentiques (notamment car theta peut être majoré unfi) par contre le second point change et il faut être un tout petit plus précis.}

\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "supp"
%%% End:


==> langevin_proof.tex <==
%\section{Proofs}
%\label{sec:contraction-properties}

%\subsection{Contraction properties}

% We introduce the following assumption on a family of Markov kernel $\{Q_{\gamma}

% We say that a family Markov kernel $Q$ on $\rset^d \times \mcb{\rset^d}$
% satisfies a Foster-Lyapunov drift condition if there exists 


%\subsection{Higher order controls}
% The next proposition is a quantitative version of \cite[Theorem 4]{brosse2018diffusion}




%\valentin{remarks sur Poisson, Wasserstein}

%\valentin{donner le quantitatif}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> results.tex <==
\subsection{SOUL method - Increasing batch size}
\label{sec:soul-method}
In this section, we consider the general setting in which $f$ is an objective function to be minimized.
In \Cref{sec:eb-inference-based}, $f(\theta) = \log(p(y | \theta))$.
We consider the following assumptions on $\Theta$ and $f$, where $\Theta \subset \rset^m$.

\begin{assumption}
  \label{assum:theta_compact}
  $\Theta$ is a convex compact set and $\Theta \subset \boulefermee{0}{M_{\Theta}}$ with $M_{\Theta}>0$.
\end{assumption}

%As regards to the function $f$ we consider the following assumptions.

\begin{assumption}
  \label{assum:f_diff}
  There exist an open set $\msu \subset \rset^m$ and $\L \geq 0$ such that $\Theta \subset \msu$ and $f \in \rmc^1(\msu,\R)$ is convex and for any $\theta_1, \theta_2 \in \Theta$
  \begin{equation}
%    \label{eq:glip_theta}
    \| \nabla f (\theta_1) - \nabla f (\theta_2) \| \leq \L \| \theta_1 - \theta_2 \| \eqsp .
  \end{equation}
  \end{assumption}
  Note that under \Cref{assum:theta_compact} and \Cref{assum:f_diff}, $\argmin_{\Theta} \ f$ is non-empty. The following assumption ensures that the gradient of the objective function can
  be written as the expectation of some integrable function.
\begin{assumption}%[\note{$V$}]
  \label{assum:grad_expec}
  For any $\theta \in \Theta$, there exist $H_{\theta}: \ \rset^d \ \rightarrow \ \rset^{d_{\Theta}}$ and a probability distribution $\pi_{\theta}$ on $(\rset^d, \mcbb(\rset^d))$ satisfying that
  % \begin{equation}
  %   \nabla f(\theta) = \left. \int_{\rset^d} H_{\theta}(x) \rme^{-U(\theta, x)} \rmd x \middle/ \int_{\rset^d} \rme^{-U(\theta, x)}\rmd x \right.\eqsp ,
  % \end{equation}
  $\pi_{\theta}(H_{\theta})< \plusinfty$ and for any $\theta \in \Theta$,
  \begin{equation}
    \label{eq:grad_def}
    \nabla_{\theta}f(\theta) = \int_{\rset^d} H_{\theta}(x) \rmd \pi_{\theta}(x) \eqsp .
  \end{equation}
In addition, $(\theta, x) \mapsto H_{\theta}(x)$ is measurable.
\end{assumption}
In \Cref{sec:eb-inference-based}, $H_{\theta}$ is given for any $\theta \in \Theta$ and $x \in \rset^d$ by $H_{\theta}(x) = \nabla_{\theta} \log(p(x,y | \theta))$, using Fisher' identity. We consider the following assumption on the family of probability distributions $(\pi_{\theta})_{\theta \in \Theta}$.
\begin{assumptionL}
  \label{assum:glip}
  For any $\theta \in \Theta$, there exists $U_{\theta}: \rset^d \to \rset$ such that $\pi_{\theta}$ admits a probability density function \wrt \ to the Lebesgue measure proportional to $x \mapsto \exp(-U_{\theta}(x))$.
  In addition $(\theta, x) \mapsto U_{\theta}(x)$ is continuous, $x \mapsto U_{\theta}(x)$ is differentiable for all $\theta \in \Theta$ and there exists $\LUx \geq 0$ such that for any $x,y \in \rset^d$,
  \begin{equation}
    \sup_{\theta \in \Theta}       \norm{\nabla_x U_{\theta}(x) -\nabla_x U_{\theta}(y)} \leq \LUx \norm{x-y} \eqsp ,
  \end{equation}
  and $\ensemble{\| \nabla_x U_{\theta}(0) \|}{\theta \in \Theta}$ is bounded.
  %on $(\rset^d, \scrB(\rset^d))$ satisfying \eqref{eq:grad_def},
%   % \begin{equation}
%   %   \nabla f(\theta) = \left. \int_{\rset^d} H_{\theta}(x) \rme^{-U(\theta, x)} \rmd x \middle/ \int_{\rset^d} \rme^{-U(\theta, x)}\rmd x \right.\eqsp ,
%   % \end{equation}
% $(\theta, x) \mapsto H_{\theta}(x)$ is measurable and $H_{\theta}$ is $\pi_{\theta}$-integrable.
\end{assumptionL}
%  \begin{assumption}
%    \label{assum:glip}
%  There exists a continuous function $U: \ \rset^d \times \Theta \to \rset$ such that for any $\theta \in \Theta$, $\int_{\rset^d} \rme^{-U(x, \theta)} \rmd x < +\infty$ and $\pi_{\theta}$ . In addition $x \mapsto U(x, \theta)$ is differentiable for all $\theta \in \Theta$ and there exists $L \geq 0$ such that for any $x,y \in \rset^d$,
%   \begin{equation}
%     \sup_{\theta \in \Theta}       \norm{\nabla_x U(x,\theta) -\nabla_x U(y,\theta)} \leq L \norm{x-y} \eqsp.
%   \end{equation}
% \end{assumption}
% \valentin{on bougera ce bout là plus tard plus haut dans l'intro de l'algo}
Once again, in \Cref{sec:eb-inference-based}, $U_{\theta}$ is given for any $\theta \in \Theta$ and $x \in \rset^d$ by $U_{\theta}(x) = -\log(p(x|y, \theta))$.
 In this context, the recursion step in \Cref{alg:souk} can be rewritten for any $n \in \N$ and $k \in \lbrace 0, \dots, m_n -1 \rbrace$
 \begin{equation}
   \begin{aligned}
 X_{k+1}^n &= X_k^n - \gamma_n \nabla_x U_{\theta_n}(X_k^n) + \sqrt{2\gamma_n} Z_{k+1}^n  \eqsp, \text{ with  $X_0^n = X_{m_{n-1}}^{n-1}$ if $n \geq 1$ }\eqsp,  \label{eq:langevin_discrete}  \\
      \theta_{n+1} &= \Pi_{\Theta}\parentheseDeux{\theta_n - m_n^{-1} \sum_{k=1}^{m_n}H_{\theta_n}(X_k^n)     }
     \end{aligned}
\end{equation}
given $(\gamma_n)_{n \in \N} \in \ocint{0,\bgamma}^{\nset}$, $(m_n)_{n \in \N} \in \left(\nsets\right)^{\N}$ and $(Z_k^n)_{n \in \N, k \in \lbrace 1, \dots, m_n \rbrace}$ a family of \iid~$d$-dimensional zero-mean Gaussian random variables with covariance matrix identity. Consider one of the following additional tail conditions on $U_{\theta}$ to ensure geometric ergodicity for the Markov chain $(X_{k}^n)_{k \in \{0,\ldots,m_n\}}$ if $\gamma_n$ is sufficiently small.


% we can use a particular case of the Markov chain defined in \eqref{eq:algo_SOUL}: the Langevin process, \ie \ for all $\theta \in \Theta$, $x \in \rset^d$ the Markov kernel $K_{\gamma, \theta}$ in \Cref{alg:souk} is given by the following Gaussian kernel $R_{\gamma, \theta}$,

% The Markov chain introduced in \eqref{eq:langevin_discrete} is a discretized version of the diffusion process defined by
% \begin{equation}
%   \label{eq:langevin_continuous}
%   \rmd X_t = - \nabla_x U_{\theta}(X_t) \rmd t + \sqrt{2} \rmd B_t \eqsp ,
% \end{equation}

\begin{assumptionL}
  \label{assum:curvature}
  There exist $\kappaun >0$ and $\kappadeux,\ccur, \Run \geq 0$ such that  for any $\theta \in \Theta$ and $x \in \rset^d$,
  % \begin{enumerate}[label=(\roman*)]
  % \item \label{assum:curvature_i}
  \[ \langle \nabla_xU_{\theta}(x), x \rangle \geq\kappaun \| x \| \1_{\boule{0}{\Run}^{\complementary}}(x) + \kappadeux \| \nabla_x U_{\theta} (x) \|^2 - \ccur\eqsp.\]
%       \item \label{assum:curvature_ii}
%     \begin{equation}
%     \langle \nabla_x U_{\theta}(x), x \rangle \geq \kappaun \| x \|^2 \1_{\boulefermee{0}{M_{\kappaun}}^{\complementary}}(x) - \ccur \eqsp.
%   \end{equation}
% \end{enumerate}
\end{assumptionL}
\valentin{non. Toujours le problème du gradient} Note that \Cref{assum:curvature} holds  if \Cref{assum:glip} does and there exist $\teta>0$, $\tc \geq 0$ such that   for any for any $\theta \in \Theta$ and $x \in \rset^d$,
    \begin{equation}
    \langle \nabla_x U_{\theta}(x), x \rangle \geq \teta \| x \|^2  - \tc \eqsp.
  \end{equation}
% Note that for any $\theta \in \Theta$ and $x \in \rset^d, \ \| x \| \geq\max( M_{\kappaun}, \kappaun / c)$ we have sub-linearity of the gradient, \ie \ $\| \nabla_x U_{\theta}(x,\theta) \| \leq(1/m) \| x \|$.
We can also derive that \Cref{assum:curvature} holds under the following assumption for $\mttdeux \geq 0$.
\begin{assumptionL}[$\mttdeux$]
  \label{assum:cvx}
  For any $\theta \in \Theta$, $U_{\theta}$ is $\mttdeux$-convex, continuously differentiable and
  \begin{equation}
    \sup_{\theta \in \Theta} \int_{\rset^d} \exp(-U_{\theta}(x)) \mathrm{d}x < +\infty \eqsp .
  \end{equation}
  In addition, $\ensemble{y \in \rset^d}{\text{there exists } \theta \in \Theta, \ \nabla_xU_{\theta}(y) = 0} \subset \ball{0}{\Rstar}$ with $\Rstar \geq 0$.
\end{assumptionL}
Note that $\ensemble{y \in \rset^d}{\text{there exists } \theta \in \Theta, \ \nabla_xU_{\theta}(y) = 0}$ is the set of minimizers of the family of functions $(U_{\theta})_{\theta \in \Theta}$.

%The following result shows that \Cref{assum:cvx}[$0$] implies that the
\begin{proposition}
\label{propo:cvx_implies_tail_condition}
  Assume  \tup{\Cref{assum:theta_compact}}, \tup{\Cref{assum:glip}} and \tup{\Cref{assum:cvx}$(0)$}. Then \tup{\Cref{assum:curvature}} holds with $\kappadeux \leftarrow 1/(4\Ltt)$.
\end{proposition}
\begin{proof}
  The proof is postponed to \Cref{sec:proof-crefpr}.
\end{proof}
While \Cref{propo:cvx_implies_tail_condition} shows that \Cref{assum:cvx}$(0)$ and additional assumptions imply  \Cref{assum:curvature}, it does not give an explicit expression for the constants appearing in this latter condition.
The next theorem asserts the convergence of the SOUL algorithm.
% scheme defined by  \eqref{eq:algo_SOUL} and \eqref{eq:langevin_discrete} referred to as the Stochastic Optimization with Unadjusted Langevin (SOUL) algorithm. % The appendix is devoted to the proof of \Cref{thm:salem_langevin_cv}, \Cref{thm:salem_langevin_bound} and \Cref{thm:salem_langevin_cv_fixed}.

% \valentin{changer le m n dans nsets et pas nset}
 \begin{theorem}
   \label{thm:salem_langevin_cv}
    Assume \tup{\Cref{assum:theta_compact}}, \tup{\Cref{assum:f_diff}}, \tup{\Cref{assum:grad_expec}} and  there exists $M_H \geq 0$ such that for any $\theta \in \Theta$ and $x \in \rset^d$, $ \| H_{\theta}(x) \| \leq M_H V^{1/2}(x)$, with \valentin{préciser V}.
    In  addition, assume \tup{\Cref{assum:glip}} and \tup{\Cref{assum:curvature}}. Set $\bgamma = \min(1,2\kappadeux) $.
Then, for all  sequences of non-increasing positive real numbers $(\gamma_n)_{n \in \nset}$,
   $(\delta_n)_{n \in \nsets}$   and  sequence of positive integers $(m_n)_{n \in \nset}$, satisfying $\sup_{n \in \nset} \gamma_n < \bgamma$,  % \Cref{assum:condition_majo_V} and \Cref{assum:condition_majo_V2} hold with $\Psibf(\gamma) = C_1 \gamma^{1/2}$ and $\Deltabf(\gamma, m)= C_2m^2$ for $C_1,C_2 \geq 0$.
% \valentin{modif}
Then, the following statements hold,
\begin{itemize}
  \item there exists $(A_n)_{n \in \nset}$ such that for any $n \in \nset$,
      \begin{equation}
%    \label{eq:L1_speed}
    \expe{  \defEns{\left. \sum_{k=1}^n \delta_k f(\theta_k) \middle/ \sum_{k=1}^n \delta_k \right. } - \min_{\Theta} f  }\leq  \left. A_n \middle/  \left( \sum_{k=1}^n \delta_k \right) \right. \eqsp ,
  \end{equation}
where \valentin{a preciser}
  \begin{multline}
A_n =  2M_{\Theta}^2 + 2M_{\Theta}\expe{V(X_0^0)} \parentheseDeux{ \frac{(A_1\vee 1) A_2 }{\rho^{\bgamma} \log(1/\rho)} \sum_{k=0}^{n} \frac{\delta_{k+1}}{ \gamma_k m_k} +    \sum_{k=0}^{n} \delta_{k+1} \Psibf(\gamma_k) } \\ +  \expe{V(X_0^0)}  \sum_{k =0}^{n} (\delta_{k+1}/m_k)^2 \Deltabf(\gamma_k, m_k)   \eqsp . \numberthis     \label{eq:horrible_bound}
\end{multline}
\item If we have 
  \begin{equation}
    \label{eq:condition_cv}
    \sum_{n=0}^{+\infty} \delta_{n+1} = +\infty \eqsp , \quad \sum_{n=0}^{+\infty} \delta_{n+1} \sqrt{\gamma_n} < +\infty \eqsp , \quad \sum_{n=0}^{+\infty} \frac{\delta_{n+1}}{ m_n \gamma_n} < +\infty \eqsp ,
  \end{equation}
then:
  \begin{enumerate}[label=(\alph*)]
  \item   $(\theta_n)_{n \in \N}$ defined by \eqref{eq:algo_SOUL} converges \as~to some $\theta^* \in \argmin_{\Theta} f$;
  \item furthermore, \as~there exists $C\geq 0$ such that for any $n \in \nsets$
  \begin{equation}
    %\label{eq:as_speed}
    \defEns{\left. \sum_{k=1}^n \delta_k f(\theta_k) \middle/ \sum_{k=1}^n \delta_k \right. } - \min_{\Theta} f \leq \left. C \middle/\left( \sum_{k=1}^n \delta_k \right) \right.  \eqsp.
  \end{equation}
\end{enumerate}
\end{itemize}
\end{theorem}


%   \begin{enumerate}[label=(\alph*)]
% \item there exists a non-negative sequence $(E_n)_{n \in \N}$ given by \eqref{eq:horrible_bound} such that for any $n \in \N$
% \begin{equation}  \expe{  \defEns{\left. \sum_{k=0}^n \delta_k f(\theta_k) \middle/ \sum_{k=0}^n \delta_k \right. } - \min_{\Theta} f  }\leq  \left. E_n \middle/  \left( \sum_{k=0}^n \delta_k \right) \right. \eqsp , \end{equation}
%   \item  in addition, assume that $(\delta_n)_{n \in \N}$, $(\gamma_n)_{n \in \N}$ and $(m_n)_{n \in \N}$ satisfy
%   \begin{equation}
%     \sum_{n=0}^{+\infty} \delta_n = +\infty \eqsp , \qquad \sum_{n=0}^{+\infty} \delta_n \gamma_n^{1/2} < +\infty \eqsp , \qquad \sum_{n=0}^{+\infty} \delta_n /(m_n \gamma_n) < +\infty \eqsp .
%   \end{equation}  $(\theta_n)_{n \in \N}$ defined by \eqref{eq:algo_SOUL} and \eqref{eq:langevin_discrete} converges \as \ to some $\theta^* \in \argmin_{\Theta} f$.
%   \item furthermore, \as~there exists $C>0$ such that
%   \begin{equation}
%     \defEns{\left. \sum_{k=0}^n \delta_k f(\theta_k) \middle/ \sum_{k=0}^n \delta_k \right. } - \min_{\Theta} f \leq \left. C \middle/\left( \sum_{k=0}^n \delta_k \right) \right.  \eqsp.
%   \end{equation}
%   \end{enumerate}


 \begin{proof}
   The proof is postponed to \Cref{sec:proof-crefthm:s-3}.
 \end{proof}

In the case  where \Cref{assum:cvx}$(m)$ with $m >0$ holds, we get the following result which implies that the bound provided by \Cref{thm:salem_cv_control} is linear in the dimension.
 \begin{corollary}% [Polynomial bounds]
   \label{thm:salem_langevin_bound}
       Assume \Cref{assum:theta_compact}, \Cref{assum:f_diff}, \Cref{assum:grad_expec} and there exists $M_H \geq 0$ such that for any $\theta \in \Theta$ and $x \in \rset^d$, $ \| H_{\theta}(x) \| \leq M_H$.
   In addition assume \Cref{assum:glip} and \Cref{assum:cvx}($\mtt$), with $\mtt>0$.
Let $\bgamma ...$ \alain{to fill}. Then, for  all  sequences of non-increasing positive real numbers $(\gamma_n)_{n \in \nset}$,
   $(\delta_n)_{n \in \nsets}$   and  sequence of positive integers $(m_n)_{n \in \nset}$, satisfying
   $\sup_{n \in \nset} \delta_n < 1/\L$, $\sup_{n \in \nset} \gamma_n < \bgamma$ and \eqref{eq:condition_cv} with $\Psibf(\gamma) = C_1 \gamma^{1/2}$, and $\Deltabf(\gamma, m)=C_2m^2$, for $C_1,C_2 \geq 0$,  the conclusions of \Cref{thm:salem_cv_control} hold with $(E_n)_{n \in \N}$ such that for any $n \in \N$, $|E_n| \leq Cd$, where $C \geq 0$ is a constant independent of the dimension $d$.
 \end{corollary}

 \begin{proof}
   The proof is postponed to \Cref{sec:proof-crefthm:s}.
 \end{proof}

 % \begin{corollary}[Polynomial bounds]
 %   \label{thm:salem_langevin_bound}
 %   Replacing \Cref{assum:curvature} or \Cref{assum:curvature2} by \Cref{assum:cvx}(m) with $m > 0$ in \Cref{thm:salem_langevin_cv}. There exist $D \in \nset$ such that \Cref{thm:salem_langevin_cv} holds for SOUL with $E_n$ a polynom in $d$ of degree lower than $D$ for any $n \in \N$.
 % \end{corollary}

 % \begin{proof}
 % \end{proof}



% \subsection{SOUPL method}
% \label{sec:soupl-method}

% Let us now consider a non-differentiable version of the SOUL method introduce in \Cref{sec:soul-method}.
% The following hypothesis is a classical splitting of $U$ into a differentiable convex function and a non-differentiable
% convex function for which a proximity operator can be computed.

% \begin{assumption}
%   \label{assum:split}
%   There exist two continuous functions $f: \rset^d \times \Theta \to \rset$, $g: \rset^d \times \Theta \to \rset$ and $L >0$ such that
%   \begin{enumerate}[label=(\alph*)]
%   \item for all $\theta \in \Theta$, $f(\cdot,\theta)$ is differentiable. In addition, for any $x, y \in \rset^d$ and $\theta \in \Theta$
%     \begin{equation}
%       \| \nabla_x f(x,\theta) - \nabla_yf(y, \theta) \| \leq L \| x - y\| \eqsp .
%     \end{equation}
%   \item $g$ is convex and $\sup_{\theta \in \Theta} \int_{\rset^d} \exp(-g(x,\theta)) \rmd x < +\infty$.
%   \end{enumerate}

%   Using the proximity operator, the algorithm in \eqref{eq:algo_SOUL} and \eqref{eq:algo_SOUL} can be rewritten for any $n \in \N$ and $k \in \lbrace 0, \dots, m_n -1 \rbrace$
% \begin{align}
%   X_{k+1}^n &= X_k^n - \gamma_n \parentheseDeux{\nabla_x U(X_k^n,\theta_n) + \lambda_n^{-1}(X_k^n - \prox_g^{\lambda}(X_k^n))}+ \sqrt{2\gamma_n} Z_{k+1}^n  \eqsp, \numberthis \label{eq:soupl} \\ &\phantom{aaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaa} \text{ with  $X_0^n = X_{m_{n-1}}^{n-1}$ if $n \geq 1$ }\eqsp,  \\
%   \theta_{n+1} &= \Pi_{\Theta}\parentheseDeux{\theta_n - \delta_n \sum_{k=1}^{m_n} H_{\theta_k}(X_k^n)} \eqsp ,
% \end{align}


%  \begin{theorem}[SOUPL bounds and convergence]
%    \label{thm:soupl_cv}
%     Assume \Cref{assum:theta_compact}, \Cref{assum:f_diff} and \Cref{assum:grad_expec}.  Let $\bgamma>0$, $(\gamma_n)_{n \in \nset}$,
%    $(\delta_n)_{n \in \nset}$ be sequences of positive real numbers and $(m_n)_{n \in \nset}$ be a sequence of positive integers satisfying
%    $\sup_{n \in \nset} \delta_n < 1/\L$, $\sup_{n \in \nset} \gamma_n < \bgamma$ and \eqref{eq:condition_cv} with $\alpha =1/2$.
%    In addition assume \Cref{assum:split} and \Cref{assum:curvature}(f) or  \Cref{assum:curvature2}(f).
%    Then \eqref{eq:condition_V} holds with $B(\gamma, \lambda) = \gamma^{1/2} + \lambda$.
%  \end{theorem}

%  \note{
%    \begin{enumerate}
%    \item écrire le lemme de la proba finie
%    \item prolonger la proposition 12 pour qu'elle gère le cas de MYULA ATTENTION LES CONSTANTES NE DOIVENT PAS DÉPENDRE DE LAMBDA
%    \item
%    \end{enumerate}
% }

 % \begin{corollary}[Polynomial bounds]
 %   \label{thm:soupl_bound}
 %   Replacing \Cref{assum:curvature} or \Cref{assum:curvature2} by \Cref{assum:cvx}(m) with $m\geq0$, \Cref{thm:salem_langevin_cv} holds with $(E_n)_{n \in \N}$ such that for any $n \in \N$, $E_n$ is a polynom in $d$.
 % \end{corollary}
 % \valentin{j'ai enlevé le théorème sur les bornes polynomiales puisqu'on supposait de la forte convexité. Je peux
 %   le remettre éventuellement... Il faudrait en fait des conditions plus fortes sur $g$}


%\end{assumption}


\subsection{SOUL method -- Fixed batch size}


 \begin{assumptionL}
  \label{assum:glip_theta}
There exists $L_{U} \geq 0$ such that for any $x\in \rset^d$ and $\theta_1, \theta_2 \in \Theta$
  \begin{equation}
  \norm{\nabla_x U_{\theta_1}(x) -\nabla_x U_{\theta_2}(x)} \leq L_U \| \theta_1 - \theta_2 \| V(x)^{1/2} \eqsp.
  \end{equation}
\end{assumptionL}

 \begin{theorem}
   \label{thm:salem_langevin_cv_fixed}
   Assume \Cref{assum:theta_compact}, \Cref{assum:f_diff}, \Cref{assum:grad_expec} and  \Cref{assum:H_lip}.    In addition assume \Cref{assum:glip}, \Cref{assum:glip_theta} and \Cref{assum:curvature}.
   Then, \Cref{assum:condition_kernel_fix} and \Cref{assum:ergo} hold with $\bgamma ...$ if , $\bgamma...$ otherwise and
   \begin{equation}
 \Lambdabf_1(\gamma_1, \gamma_2) = (\gamma_2^{-1} - \gamma_1^{-1})^{1/2} + \gamma_2^{-1/2}\abs{\gamma_1 - \gamma_2} \eqsp , \qquad \Lambdabf_2(\gamma_1, \gamma_2) \leq \gamma_2^{1/2} \eqsp ,
   \end{equation}
 \end{theorem}

 \begin{proof}
   The proof is postponed to \Cref{sec:proof-crefthm:s-1}.
 \end{proof}


 \valentin{modif}

In this section, we consider the case where the batch size is fixed, \ie \ $m_n = m_0$ for all $n \in \nset$. For ease of exposition we only consider the case where $m_0 = 1$. However the general case can be adapted from the proof of the result stated below. For ease of notation, we let $\tX_{n+1} = X_1^n$ for any $n \in \nset$. More precisely the recursion \eqref{eq:algo_SOUL} and \eqref{eq:algo_SOUL} can be written for any $n \in \nset$ as
\begin{equation}
   \label{eq:algo_x_fix}
\begin{aligned}
  & \X_{n+1} \text{ has distribution } K_{\gamma_n, \ttheta_n}(\X_n, \cdot) \text{ conditionally to } \F_{n} \eqsp , \\
  %\X_{n+1}^n &\sim K_{\gamma_n, \ttheta_n}(\X_n^n, \cdot)  \eqsp, \text{ with  $\X_0^n = \X_{m_{n-1}}^{n-1}$ if $n \geq 1$ }\eqsp, \\
  &\ttheta_{n+1} = \Pi_{\Theta}\parentheseDeux{\ttheta_n - \delta_{n+1} H_{\ttheta_n}(\X_{n+1})} \eqsp ,
\end{aligned}
\end{equation}
with $\theta_0 \in \Theta$, $\tX_0 \in \rset^d$ random variables and where  $\F_n$ is given by
\begin{equation}
  \label{eq:def_tmcf}
  \F_n = \sigma \left( \ttheta_0, (\X_{\ell})_{\ell \in \{0,\ldots,n\}} \right) \eqsp.
\end{equation}
We consider the following additional assumptions.
% We rewrite \eqref{eq:algo_SOUL} and \eqref{eq:algo_SOUL}. Starting from $X_0 \in \rset^d$ and $\ttheta_0 \in \ttheta$ we define $(X_k, \ttheta_k)_{k \in \N}$ by the following recursion
% \begin{align}
%     \label{eq:algo_SOUL_fix}
%   X_{k+1} &\sim K_{\gamma_n, \ttheta_n}(X_k, \cdot)  \eqsp,  \\
%   \label{eq:algo_SOUL_fix}
%   \ttheta_{k+1} &= \Pi_{\ttheta}\parentheseDeux{\ttheta_k -  \delta_{k+1} H_{\ttheta_n}(X_{k+1})} \eqsp ,
                    %   \end{align}
%We impose some Lipschitz-regularity over $(\theta, x) \mapsto H_{\theta}(x)$.
\begin{assumption}
  \label{assum:H_lip}
  There exist a measurable function $V : \rset^d \to \coint{1,\plusinfty}$ and $M_H,L_H \geq 0$ such that for any $x \in \rset^d$ and $\theta_1, \theta_2 \in \Theta$,
  \begin{equation}
    \| H_{\theta_1}(x) - H_{\theta_2}(x) \| \leq L_H \| \theta_1 - \theta_2\| V^{1/2}(x) \eqsp , \qquad  \norm{H_{\theta_1}(x)} \leq M_H V^{1/4}(x) \eqsp .
  \end{equation}
\end{assumption}

\begin{assumptionH}
  \label{assum:condition_majo_V_fix_}
  There exists a measurable function $V : \rset^d \to \coint{1,\plusinfty}$
  and $ A_3 \geq 0$ such that for any $n \in \N$
       \begin{equation}
     \label{eq:condition_majo_V_fix}
     \CPE{V(\tX_{n})}{\tX_0} \leq A_3 V(\tX_0) \eqsp , \qquad \expe{V(\tX_0)} < + \infty \eqsp,
   \end{equation}
   where $(\tX_n)_{n \in \nset}$ is defined by \eqref{eq:algo_x_fix}.
  % In addition, there exist $\bgamma >0$, $A_2,  \geq 0$, $B: \R_+^*\to \R_+$ such that for any $\gamma \in\ocint{0,\bgamma}$, $\theta \in \Theta$, $x \in \rset^d$ and  $n \in \N$
  %  \begin{equation}
  %    \label{eq:condition_V_fix}
  %    \abs{\int_{\rset^d} K_{\gamma, \theta}^n(x, \rmd y) H_{\theta}(y) - \pi_{\theta} (H_{\theta})} \leq A_2 \rho^{n \gamma}V(x) + \Psibf(\gamma) \eqsp .
  %  \end{equation}
 \end{assumptionH}
% \begin{assumption}
%   \label{assum:condition_majo_V_fix}
%   % Let $(\X_n, \ttheta_n)_{n \in \N}$ be given by \eqref{eq:algo_x_fix} and \eqref{eq:algo_theta_fix}.
%   There exists $A_1 \geq 0$ such that for any $n \in \N$
%        \begin{equation}
%      \qquad \CPE{V(\X_{n})}{\X_0} \leq A_1 V(\X_0) \eqsp , \qquad \expe{V(\X_0)} < + \infty \eqsp ,
%    \end{equation}

%  \end{assumption}
We consider a similar property as \Cref{assum:H_lip} on the family of kernels $\defEns{ K_{\gamma, \theta}, \gamma \in\ocint{0,\bgamma}, \theta \in \Theta }$, , which weakens the assumption \cite[H6]{atchade2017perturbed}.

\begin{assumptionH}
  \label{assum:condition_kernel_fix}
  There exist  $\Lambdabf_1: \left( \rset_+^* \right)^2 \to \rset_+$ and $\Lambdabf_2: \left( \rset_+^* \right)^2 \to \rset_+$ such that for any $\gamma_1,\gamma_2 \in\ocint{0,\bgamma}$ , $\theta_1,\theta_2 \in \Theta$, $x \in \rset^d$
  and $a \in \ccint{1/4, 1/2}$
        \begin{equation}
     \Vnorm[V^{a}]{\updelta_x K_{\gamma_1, \theta_1} - \updelta_x K_{\gamma_2, \theta_2} } \leq \parentheseDeux{ \Lambdabf_1(\gamma_1, \gamma_2)  + \Lambdabf_2(\gamma_1, \gamma_2)\| \theta_1 - \theta_2 \| } V^{2a}(x) \eqsp .
   \end{equation}

\end{assumptionH}


Finally, we suppose that each kernel $K_{\gamma, \theta}$ admits an invariant probability measure and converges geometrically to this probability distribution in $V$-norm with constants not depending on $\gamma$ and $\theta$. We show in \cite{debortoli2018back} that this condition holds for the Langevin Monte Carlo algorithm. % It has been shown
% that various Markov chains satisfy this assumption, see \cite{brosse2018diffusion} for example\valentin{back}.

\begin{assumptionH}
  \label{assum:ergo}
  For all $\theta \in \Theta$ and $\gamma \in\ocint{0,\bgamma}$ , $K_{\gamma, \theta}$ is uniformly $V$-geometrically ergodic, \ie \ there exists a probability distribution $\pi_{\gamma, \theta}$ on $(\rset^d, \scrB(\rset^d))$, $A_4 \geq 0$ and $\kappa \in (0,1)$ such that for any $n \in \N$ and $a \in \ccint{1/4,1}$
  \begin{equation}
    \Vnorm[V^{a}]{ K_{\gamma, \theta}^n - \pi_{\gamma, \theta}} \leq A_4 \kappa^{n \gamma} V^{a}(x) \eqsp .
  \end{equation}
\end{assumptionH}


The following theorem ensures convergence properties for the algorithm similar to \Cref{thm:salem_cv}.
The proof of this result is based on  a generalization of \cite[Lemma 4.2]{fort2011convergence}, which only holds in the case of exact MCMC schemes.
\begin{theorem}
  \label{thm:salem_cv_fix}
  Assume \Cref{assum:theta_compact}, \Cref{assum:f_diff}, \Cref{assum:grad_expec} and \Cref{assum:H_lip}.
  Let $\bgamma>0$, $(\gamma_n)_{n \in \nset}$ and
   $(\delta_n)_{n \in \nsets}$ be sequences of non-increasing positive real numbers satisfying
   $\sup_{n \in \nset} \delta_n < 1/\L$, $\sup_{n \in \nset} \gamma_n < \bgamma$,   $ \sup_{n \in \N} |\delta_{n+1} - \delta_n | \delta_n^{-2} < +\infty$,  $\sum_{n=0}^{+\infty} \delta_{n+1} = +\infty$ and
  \begin{equation}
    \label{eq:condition_cv_fix_1}
      \sum_{n=0}^{+\infty} \delta_{n+1} \Psibf(\gamma_n) < +\infty \eqsp , \ \sum_{n=0}^{+\infty} \frac{\delta_{n+1}^2}{\gamma_n^2}  < +\infty \eqsp , \
    \sum_{n=0}^{+\infty} \frac{\delta_{n+1}}{\gamma_{n+1}} \parentheseDeux{ \Lambdabf_1(\gamma_n, \gamma_{n+1}) +  \delta_{n+1} \Lambdabf_2(\gamma_n, \gamma_{n+1})}  < +\infty \eqsp .
  \end{equation}
  Let $(\X_n)_{n \in \N}$ be given by \eqref{eq:algo_x_fix}.
    Assume in addition that  \Cref{assum:condition_majo_V}-\ref{assum:condition_majo_V_ii}, \Cref{assum:condition_majo_V_fix_},  \Cref{assum:condition_kernel_fix}, \Cref{assum:ergo} hold.
  Then the following statements hold:
  \begin{enumerate}[label=(\alph*)]
  \item   $(\ttheta_n)_{n \in \N}$ defined by \eqref{eq:algo_x_fix} converges \as~to some $\theta^* \in \argmin_{\Theta} f$;
  \item furthermore, \as~there exists $C\geq0$ such that for any $n \in \nsets$
  \begin{equation}
    \defEns{\left. \sum_{k=1}^n \delta_k f(\ttheta_k) \middle/ \sum_{k=1}^n \delta_k \right. } - \min_{\Theta} f \leq \left. C \middle/\left( \sum_{k=1}^n \delta_k \right) \right.  \eqsp.
  \end{equation}
  \end{enumerate}
\end{theorem}


\begin{proof}
  The proof of this theorem is postponed to \Cref{sec:proof-crefthm:s-2}.
\end{proof}

% \begin{proof}
%   The
% \end{proof}
                    %                     The proof of this theorem is postponed to the supplementary paper \cite[Theorem]{debortoli2018souk_supplementary} \valentin{thm cv}.

In our case of application $\Psibf(\gamma) = C_1\gamma^{1/2}$, $\Lambdabf_1(\gamma_1, \gamma_2) =  C_2 (\gamma_2^{-1} - \gamma_1^{-1})^{1/2} + \gamma_2^{-1/2}\abs{\gamma_1 - \gamma_2}$ and $\Lambdabf_2(\gamma_1, \gamma_2) = C_3\gamma_2^{1/2}$, for $C_1,C_2,C_3 \geq 0$. Thus we obtain that the following series should be convergent
  \begin{equation}
     \sum_{n=0}^{+\infty} \delta_{n+1}\gamma_n^{1/2} < +\infty \eqsp , \quad \sum_{n=0}^{+\infty} \delta_{n+1}^2 / \gamma_n^2  < +\infty \eqsp , \quad \sum_{n=0}^{+\infty} \delta_{n+1} (\gamma_{n+1}^{-1} - \gamma_{n}^{-1})^{1/2} / \gamma_n^2  < +\infty \eqsp .
   \end{equation}
   A possible choice is given $\delta_n = n^{-1}$ and $\gamma_n = \log(n+1)^{-4}$. In this setting it should be noted that the sequence of $(\ttheta_n)_{n \in \nset}$ moves slowly compared to the sequence $(\tX_n)_{n \in \N}$. In the limiting case, if we suppose that $\ttheta_n$ is constant we obtain that averaging the sequence $(\tX_n)_{n \in \N}$ is an estimator of $\nabla f(\ttheta_n)$. This is coherent with the increasing batch size approach.

% In our case of application $\Psibf(\gamma) = E(\gamma) = \gamma^{1/2}$
% A possible choice for the sequence $(\delta_n)_{n \in \nsets}$ and $(\gamma_n)_{n \in \N}$ is then given by
% $\delta_n = n^{-1}$ and $\gamma_n = \log(n)^{-4}$.











%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main_jrssb"
%%% End:

